Preventing Collapse in Contrastive Learning with Orthonormal Prototypes (CLOP)

Contrastive learning has emerged as a powerful method in deep learning, excelling at learning effective representations through contrasting samples from different distributions. However, neural collapse, where embeddings converge into a lower-dimensional space, poses a significant challenge, especially in semi-supervised and self-supervised setups. In this paper, we first theoretically analyze the effect of large learning rates on contrastive losses that solely rely on the cosine similarity metric, and derive a theoretical bound to mitigate this collapse. {Building on these insights, we propose CLOP, a novel semi-supervised loss function designed to prevent neural collapse by promoting the formation of orthogonal linear subspaces among class embeddings.} Unlike prior approaches that enforce a simplex ETF structure, CLOP focuses on subspace separation, leading to more distinguishable embeddings. Through extensive experiments on real and synthetic datasets, we demonstrate that CLOP enhances performance, providing greater stability across different learning rates and batch sizes.

==> raw-tables.tex <==
\clearpage
\subsection{Semi-Supervised Learning with $50\%$ Labels}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Batch size} &\textbf{32} &\textbf{64} &\textbf{128} &\textbf{256} &\textbf{512} &\textbf{1024} &\textbf{2048} \\ \hline
InfoNCE-OAR on Cifar100 &0.601 &0.648 &0.664 &0.683 &0.703 &0.665 &0.634\\ \hline
InfoNCE on Cifar100 &0.524 &0.517 &0.554 &0.581 &0.591 &0.595 &0.606\\ \hline
InfoNCE-OAR on Tiny-ImageNet &0.620 &0.662 &0.679 &0.695 &0.708 &0.691 &0.679\\ \hline
InfoNCE on Tiny-ImageNet &0.452 &0.465 &0.477 &0.487 &0.482 &0.475 &0.485\\ \hline
\end{tabular}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Batch size} &\textbf{32} &\textbf{64} &\textbf{128} &\textbf{256} &\textbf{512} &\textbf{1024} &\textbf{2048} \\ \hline
InfoNCE-OAR on Cifar100 &0.868 &0.892 &0.874 &0.894 &0.903 &0.904 &0.891\\ \hline
InfoNCE on Cifar100 &0.813 &0.814 &0.841 &0.857 &0.865 &0.865 &0.874\\ \hline
InfoNCE-OAR on Tiny-ImageNet &0.864 &0.887 &0.890 &0.91 &0.91 &0.9 &0.891\\ \hline
InfoNCE on Tiny-ImageNet &0.715 &0.733 &0.746 &0.747 &0.747 &0.743 &0.747\\ \hline
\end{tabular}
\caption{Top-1/Top-5 accuracy vs batch size. Learning Rate of 0.3*batch size/256}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Learning rate} &\textbf{0.1} &\textbf{0.8} &\textbf{1.2} &\textbf{1.6} &\textbf{2.0} &\textbf{2.4} &\textbf{2.8} &\textbf{10} \\ \hline
InfoNCE-OAR on Cifar100 &0.478 &0.649 &0.664 &0.656 &0.669 &0.665 &0.638 &0.606\\ \hline
InfoNCE on Cifar100 &0.458 &0.583 &0.601 &0.611 &0.601 &0.595 &0.582 &0.477\\ \hline
InfoNCE-OAR on Tiny-ImageNet &0.442 &0.704 &0.691 &0.673 &0.633 &0.604 &0.598 &0.577\\ \hline
InfoNCE on Tiny-ImageNet &0.411 &0.479 &0.475 &0.475 &0.467 &0.468 &0.468 &0.275\\ \hline
\end{tabular}

\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Learning rate} &\textbf{0.1} &\textbf{0.8} &\textbf{1.2} &\textbf{1.6} &\textbf{2.0} &\textbf{2.4} &\textbf{2.8} &\textbf{10} \\ \hline
InfoNCE-OAR on Cifar100 &0.771 &0.894 &0.902 &0.906 &0.906 &0.904 &0.889 &0.87\\ \hline
InfoNCE on Cifar100 &0.756 &0.86 &0.874 &0.876 &0.87 &0.865 &0.859 &0.774\\ \hline
InfoNCE-OAR on Tiny-ImageNet &0.707 &0.912 &0.9 &0.869 &0.854 &0.838 &0.834 &0.837\\ \hline
InfoNCE on Tiny-ImageNet &0.672 &0.747 &0.743 &0.742 &0.734 &0.731 &0.720 &0.538\\ \hline
\end{tabular}
\caption{Top-1/Top-5 accuracy vs lr. Batch size of 1024}
\end{table}


\clearpage
\subsection{Semi-Supervised Learning with $10\%$ Labels (only on Tiny-Imagenet)}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Batch size} &\textbf{32} &\textbf{64} &\textbf{128} &\textbf{256} &\textbf{512} &\textbf{1024} &\textbf{2048} \\ \hline
InfoNCE-OAR on Tiny-ImageNet &0.554 &0.592 &0.615 &0.636 &0.646 &0.643 &0.648\\ \hline
InfoNCE on Tiny-ImageNet &0.454 &0.462 &0.476 &0.475 &0.475 &0.473 &0.481\\ \hline
\end{tabular}
% \caption{Top-1 accuracy vs batch size.}
% \end{table}


% \begin{table}[h]
% \centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Batch size} &\textbf{32} &\textbf{64} &\textbf{128} &\textbf{256} &\textbf{512} &\textbf{1024} &\textbf{2048} \\ \hline
InfoNCE-OAR on Tiny-ImageNet &0.823 &0.847 &0.866 &0.883 &0.883 &0.883 &0.889\\ \hline
InfoNCE on Tiny-ImageNet &0.722 &0.729 &0.742 &0.74 &0.74 &0.74 &0.748\\ \hline
\end{tabular}
\caption{Top-1/Top-5 accuracy vs batch size. Learning Rate of 0.3*batch size/256}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Learning rate} &\textbf{0.1} &\textbf{0.8} &\textbf{1.2} &\textbf{1.6} &\textbf{2.0} &\textbf{2.4} &\textbf{2.8} &\textbf{10} \\ \hline
InfoNCE-OAR on Tiny-ImageNet &0.424 &0.638 &0.643 &0.647 &0.644 &0.631 &0.624 &0.507\\ \hline
InfoNCE on Tiny-ImageNet &0.413 &0.476 &0.473 &0.469 &0.465 &0.463 &0.455 &0.276\\ \hline
\end{tabular}
% \caption{Top-1 accuracy vs lr.}
% \end{table}

% \begin{table}
% \centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Learning rate} &\textbf{0.1} &\textbf{0.8} &\textbf{1.2} &\textbf{1.6} &\textbf{2.0} &\textbf{2.4} &\textbf{2.8} &\textbf{10} \\ \hline
InfoNCE-OAR on Tiny-ImageNet &0.694 &0.884 &0.883 &0.89 &0.883 &0.876 &0.871 &0.776\\ \hline
InfoNCE on Tiny-ImageNet &0.678 &0.745 &0.740 &0.737 &0.735 &0.729 &0.72 &0.541\\ \hline
\end{tabular}
\caption{Top-1/Top-5 accuracy vs lr. Batch size of 1024}
\end{table}


\clearpage
\subsection{Fully-Supervised Learning}
\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Batch size} &\textbf{32} &\textbf{64} &\textbf{128} &\textbf{256} &\textbf{512} &\textbf{1024} &\textbf{2048} \\ \hline
SupCon-OAR on Cifar100 &0.723 &0.723 &0.696 &0.720 &0.733 &0.754 &0.746\\ \hline
SupCon on Cifar100 &0.567 &0.601 &0.666 &0.716 &0.715 &0.733 &0.734\\ \hline
SupCon-OAR on Tiny-ImageNet &0.629 &0.661 &0.683 &0.701 &0.708 &0.696 &0.659\\ \hline
SupCon on Tiny-ImageNet &0.458 &0.472 &0.482 &0.485 &0.488 &0.488 &0.504\\ \hline
\end{tabular}
% \caption{Top-1 accuracy vs batch size.}
% \end{table}

% \begin{table}[h]
% \centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Batch size} &\textbf{32} &\textbf{64} &\textbf{128} &\textbf{256} &\textbf{512} &\textbf{1024} &\textbf{2048} \\ \hline
SupCon-OAR on Cifar100 &0.927 &0.923 &0.92 &0.924 &0.927 &0.938 &0.936\\ \hline
SupCon on Cifar100 &0.846 &0.872 &0.903 &0.921 &0.922 &0.935 &0.936\\ \hline
SupCon-OAR on Tiny-ImageNet &0.865 &0.845 &0.888 &0.897 &0.906 &0.9 &0.878\\ \hline
SupCon on Tiny-ImageNet &0.721 &0.738 &0.747 &0.756 &0.759 &0.756 &0.766\\ \hline
\end{tabular}
\caption{Top-1/Top-5 accuracy vs batch size. Learning rate of 0.3*batch size/256}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Learning rate} &\textbf{0.1} &\textbf{0.8} &\textbf{1.2} &\textbf{1.6} &\textbf{2.0} &\textbf{2.4} &\textbf{2.8} &\textbf{10} \\ \hline
SupCon-OAR on Cifar100 &0.565 &0.744 &0.744 &0.749 &0.747 &0.754 &0.75 &0.657\\ \hline
SupCon on Cifar100 &0.548 &0.739 &0.745 &0.746 &0.736 &0.733 &0.720 &0.543\\ \hline
SupCon-OAR on Tiny-ImageNet &0.451 &0.703 &0.696 &0.664 &0.635 &0.622 &0.606 &0.578\\ \hline
SupCon on Tiny-ImageNet &0.419 &0.487 &0.488 &0.483 &0.477 &0.47 &0.475 &0.282\\ \hline
\end{tabular}
% \caption{Top-1 accuracy vs lr.}
% \end{table}

% \begin{table}[h]
% \centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Learning rate} &\textbf{0.1} &\textbf{0.8} &\textbf{1.2} &\textbf{1.6} &\textbf{2.0} &\textbf{2.4} &\textbf{2.8} &\textbf{10} \\ \hline
SupCon-OAR on Cifar100 &0.835 &0.929 &0.929 &0.935 &0.932 &0.938 &0.935 &0.875\\ \hline
SupCon on Cifar100 &0.832 &0.928 &0.931 &0.937 &0.931 &0.934 &0.928 &0.825\\ \hline
SupCon-OAR on Tiny-ImageNet &0.719 &0.809 &0.9 &0.878 &0.856 &0.835 &0.782 &0.853\\ \hline
SupCon on Tiny-ImageNet &0.686 &0.751 &0.756 &0.749 &0.743 &0.74 &0.74 &0.547\\ \hline
\end{tabular}
\caption{Top-1/Top-5 accuracy vs lr. Batch size of 1024}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Similarity Metric} &\textbf{Top-1 Cifar100} &\textbf{Top-5 Cifar100} &\textbf{Top-1 Tiny-Imagenet} &\textbf{Top-5 Tiny-Imagenet}\\ \hline
Cosine &0.754 &0.938 &0.595 &0.845\\ \hline
Euclidean &0.749 &0.933 &0.588 &0.839\\ \hline
Manhattan &0.715 &0.899 &0.659 &0.878\\ \hline
\end{tabular}
\caption{Accuracy of different distance method, train on SupCon-OAR. Cifar100 is trained on 1024, and Tiny-Imagenet is trained on 2048}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Augmentation} &\textbf{Top-1 Accuracy} &\textbf{Top-5 Accuracy}\\ \hline
RandAug &0.696 &0.9 \\ \hline
AutoAug-Imagenet &0.546 &0.776\\ \hline
SimCLR-like Augmentation &0.499 &0.77\\ \hline
\end{tabular}
\caption{Accuracy of different augmentation method on Tiny ImageNet. It is shown that the Random Augmentation yield the best result for both Top-1 and Top-5. The results are trained on batch size 1024.}
\end{table}
